Towards Transaction as a Service

This paper argues for decoupling transaction processing from existing two-layer cloud-native databases and making transaction processing as an independent service. By building a transaction as a service (TaaS) layer, the transaction processing can be independently scaled for high resource utilization and can be independently upgraded for development agility. Accordingly, we architect an execution-transaction-storage three-layer cloud-native database. By connecting to TaaS, 1) the AP engines can be empowered with ACID TP capability, 2) multiple standalone TP engine instances can be incorporated to support multi-master distributed TP for horizontal scalability, 3) multiple execution engines with different data models can be integrated to support multi-model transactions, and 4) high performance TP is achieved through extensive TaaS optimizations and consistent evolution. Cloud-native databases deserve better architecture: we believe that TaaS provides a path forward to better cloud-native databases.

==> 5.conclusion.tex <==

\section{Conclusions}
\label{sec:conclusion}

In this paper, we propose to decouple transaction processing from existing compute-storage disaggregated databases, resulting an execute-transaction-storage three-layer database architecture. We propose to make transaction processing an independent service, \taas, which can be independently scaled and independently evolved. We demonstrate the nice properties of \taas. By connecting to \taas, we can empower existing NoSQL databases with TP capability, make standalone TP engine support distributed TP, and support multi-model transactions in a trivial way. All the nice properties demonstrate the promising future of \taas. We will summarize the challenges and opportunities for building the ecosystem around \taas in the next version.
